Learning Embeddings with Centroid Triplet Loss for Object Identification in Robotic Grasping

Foundation models are a strong trend in deep learning and computer vision. These models serve as a base for applications as they require minor or no further fine-tuning by developers to integrate into their applications. Foundation models for zero-shot object segmentation such as Segment Anything (SAM) output segmentation masks from images without any further object information. When they are followed in a pipeline by an object identification model, they can perform object detection without training. Here, we focus on training such an object identification model. A crucial practical aspect for an object identification model is to be flexible in input size. As object identification is an image retrieval problem, a suitable method should handle multi-query multi-gallery situations without constraining the number of input images (e.g. by having fixed-size aggregation layers). The key solution to train such a model is the centroid triplet loss (CTL), which aggregates image features to their centroids. CTL yields high accuracy, avoids misleading training signals and keeps the model input size flexible. In our experiments, we establish a new state of the art on the ArmBench object identification task, which shows general applicability of our model. We furthermore demonstrate an integrated unseen object detection pipeline on the challenging HOPE dataset, which requires fine-grained detection. There, our pipeline matches and surpasses related methods which have been trained on dataset-specific data.

==> sections/tmp_abstract.tex <==
Foundation models are a strong trend in deep learning and computer vision. These models serve as a base for applications as they require minor or no further fine-tuning by developers to integrate into their applications. Foundation models for zero-shot object segmentation such as Segment Anything (SAM) output segmentation masks from images without any further object information. When they are followed in a pipeline by an object identification model, they can perform object detection without training. Here, we focus on training such an object identification model. A crucial practical aspect for an object identification model is to be flexible in input size. As object identification is an image retrieval problem, a suitable method should handle multi-query multi-gallery situations without constraining the number of input images (e.g. by having fixed-size aggregation layers). The key solution to train such a model is the centroid triplet loss (CTL), which aggregates image features to their centroids. CTL yields high accuracy, avoids misleading training signals and keeps the model input size flexible. In our experiments, we establish a new state of the art on the ArmBench object identification task, which shows general applicability of our model. We furthermore demonstrate an integrated unseen object detection pipeline on the challenging HOPE dataset, which requires fine-grained detection. There, our pipeline matches and surpasses related methods which have been trained on dataset-specific data. Code and pretrained models are available.

==> sections/trash.tex <==
% ==============================================================
% INTRODUCTION

% who applications can utilize our model
Robotic grasping in general and bin picking in specific could benefit from a generic object-matching model. Many logistics entities and retailers in industry capture image of their products. Walmart for example offers an API service to acquire images of any of the products by their product ID. Other supply chain management such as Arvato capture images of all incoming new unique products to guide workers in their picking stations \cite{}. These images represent the gallery images. Having such images empowers to enhance or develop some applications such as:
% Applications:
% Check if grasped object is correct
% mixed bin picking (very known)
% helps with crash detection (many objects there that should not be there)
% automatic inventory counting
% modern product flow (mixing orders, mixing dispatching and etc)
\begin{itemize}
    \item Verify grasped objects:
    A mistake that happens often in off-the-shelf software for bin picking is grasping dummy objects. in a realistic case, a bin can contain leftovers from product packages or empty cardboard boxes. Zero-shot segmentation would blindly segment them. A generic object-matching model with images of the product can verify if the grasped objects are correct.
    \item Mixed bin picking:
    This is a well-known application that came up in the Amazon robotics challenge \cite{}. Where many objects of different types are stored together in one bin.
    \item inventory counting and defect detection:
    The process could be automated by associating the object in the database with the real content of the bin.
    \item Mixed material flow:
    from an economical perspective and logistics process optimization, it can be cheaper or faster when multiple orders are picked together from a bin, and the flow gets separated later.
\end{itemize}

% not everyone need to train
In very recent years, computer vision foundation models started to be generic. This empowers applications to be built on top of such generic models directly. The application developer wouldn't need to train or even fine-tune the model.
These models handled different aspects of computer vision and object recognition.
% CLIP
%CLIP \cite{} made a generic text to visual representations.
% Segment Anything
The zero-shot generic segmentation Segment-Anything model (SAM) \cite{} can segment any objects in an image using point prompts. Other foundation models as FastSAM and Semantic-SAM followed.
% CNOS - SAM6D in the context to robotic grasping
Some pipeline utilized SAM to do 6D pose estimation such as CNOS \cite{} and SAM-6D \cite{}. This challenge came up last year in the BOP challenge as they introduced a new category of tasks for unseen object 6D pose, segmentation, and detection. Both pipelines followed a similar scheme. The first stage is zero-shot segmentation with SAM or similar models. The second stage is matching the segmentation masks with gallery images generated from CAD models. The third and last stage is to associate the mask or its corresponding point cloud to the CAD model to obtain the 6D pose of the object.


This matching task is defined as matching group of query images to a group of gallery images. This query gallery can be the output of zero-shot classification models such as SAM or any other application-specific method. It should be possible to use a set multiple query images per object, which could happen in some applications. The gallery images ideally should cover all the unique faces of an object. The model matches each query image/set-of-images to one, many, or none of the gallery objects.

% Object segmentation for robotic grasping is a common product, especially in bin-picking
% Some applications can utilize a generic object-matching model. As bin picking is nowadays the biggest real-world application for robotic grasping. It is so simple nowadays with many off-the-shelf software available. Some of these software are model-based and others are model-free with the model-free ones being mostly deep-learning-based generic segmentation.

% modern warehouses and companies take images of their products
% this is the query set
% Wallmart image service
% Arvato warehouses taking images of all new objects
% A model that can do generic segmentation can have many possibilities. Most modern warehouses serving different industries capture images of their new products. Some in retail companies as Walmart provide an API service to retrieve these images \cite{}. Other supply chain management such as Arvato capture images of all incoming new unique products to guide workers in their picking stations \cite{}. Having images of all products and a model that can do generic classification would help in handling or developing such new applications:
% ==============================================================
